Learning to Extract Structured Entities Using Language Models

Recent advances in machine learning have significantly impacted the field of information extraction, with Language Models (LMs) playing a pivotal role in extracting structured information from unstructured text. Prior works typically represent information extraction as triplet-centric and use classical metrics such as precision and recall for evaluation. We reformulate the task to be entity-centric, enabling the use of diverse metrics that can provide more insights from various perspectives. We contribute to the field by introducing Structured Entity Extraction and proposing the Approximate Entity Set OverlaP (AESOP) metric, designed to appropriately assess model performance. Later, we introduce a new Multistage Structured Entity Extraction (MuSEE) model that harnesses the power of LMs for enhanced effectiveness and efficiency by decomposing the extraction task into multiple stages. Quantitative and human side-by-side evaluations confirm that our model outperforms baselines, offering promising directions for future advancements in structured entity extraction. Our source code and datasets are available at https://github.com/microsoft/Structured-Entity-Extraction.

==> section/01-intro.tex <==
% \vspace{-6mm}
\section{Introduction}
\label{sec:intro}
\vspace{-2mm}
Information extraction refers to a broad family of challenging natural language processing (NLP) tasks that aim to extract structured information from unstructured text~\citep{cardie1997empirical, eikvil1999information, chang2006survey, sarawagi2008information, grishman2015information, niklaus2018survey, nasar2018information, wang2018clinical, martinez2020information}.
Examples of information extraction tasks include:
% \begin{enumerate*}[label=\textit{(\roman*)}]
%     \item Named-entity recognition~\citep{nadeau2007survey, marrero2013named, sharnagat2014named, yadav2018survey, goyal2018recent, li2020survey},
%     \item relation extraction~\citep{bach2007survey, pawar2017relation, kumar2017survey, nasar2021named},
%     \item event extraction~\citep{hogenboom2011overview, xiang2019survey, li2022survey}, and
%     \item coreference resolution~\citep{elango2005coreference, zheng2011coreference, lu2018event, sukthanker2020anaphora, stylianou2021neural, liu2023brief},
% \end{enumerate*}
\begin{enumerate*}[label=\textit{(\roman*)}]
    \item Named-entity recognition~\citep{ li2020survey},
    \item relation extraction~\citep{kumar2017survey},
    \item event extraction~\citep{li2022survey}, and
    \item coreference resolution~\citep{ stylianou2021neural, liu2023brief},
\end{enumerate*}
as well as higher-order challenges, such as automated knowledge base (KB) and knowledge graph (KG) construction from text~\citep{weikum2010information, ye2022generative, zhong2023comprehensive}.
The latter may in turn necessitate solving a combination of the former more fundamental extraction tasks as well as require other capabilities like entity linking~\citep{shen2014entity, shen2021entity, oliveira2021towards, sevgili2022neural}.
In this work, we focus on \textit{S}tructured \textit{E}ntity \textit{E}xtraction (SEE), another fundamental and challenging information extraction task and an important ingredient in automated KB construction.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{fig/example_task.png}
    \caption{Illustration of the structured entity extraction task. Given a text description as well as some predefined schema containing all the candidates of entity types and property keys, our task aims to output a structured json for all entities in the text with their information.}
    \label{fig:task}
    \vspace{-6mm}
\end{figure}

We define a structured entity as a named entity with associated properties and relationships with other named-entities.
Extracting a structured entity from unstructured text therefore \new{implicitly} combines named-entity recognition, entity-property extraction, relationship extraction, and coreference resolution.
Fig.~\ref{fig:task} shows an illustration of the structured entity extraction task.
Given a text description, we aim to first identify the two entities mentioned \textit{``Bill Gates''} and \textit{``Microsoft''}.
During this phase, we need to also address the \new{coreference resolution} and identify that \textit{``Bill Gates''} and \textit{``Gates''} are the same entity.
Then, given some predefined schema on the all possible entity types and property keys, the exact types, property keys, property values on all identified entities in the text are expected to be predicted, as well as the relations between these two entities (i.e., \textit{Bill Gates} co-founded \textit{Microsoft}).
Such extracted structured entities may be further linked and merged to automatically construct KBs from text corpora.
We present our formalization of the \textit{structured entity extraction} task which lays the foundation for evaluation for this information extraction task.
Along with this, we propose a new evaluation metric with numerous variants for measuring the similarity between the predicted set of entities and the ground truth set, which is appropriate for our task (see Sec.~\ref{sec:prelim}).





In recent years, deep learning has garnered significant interest in the realm of information extraction tasks. 
Techniques based on deep learning for entity extraction have consistently outperformed traditional methods that rely on features and kernel functions, showcasing superior capability in feature extraction and overall accuracy~\citep{yang2022survey}. 
Building upon these developments, our study employs large language models (LLMs) to tackle the challenge of structured entity extraction. 
We introduce a \textit{Mu}lti-stage \textit{S}tructured \textit{E}ntity \textit{E}xtraction (MuSEE) model, a novel architecture that enhances both effectiveness and efficiency in this task.
Our model decomposes the entire information extraction task into multiple stages, enabling parallel predictions within each stage for enhanced focus and accuracy.
Additionally, we reduce the number of tokens needed for generation, which further improves the efficiency for both training and inference.
Human side-by-side evaluations further confirm that our model's effectiveness over baselines.


% It is noteworthy that~\citet{lu2023pivoine} have also employed LLMs for zero-shot structured entity extraction. 
% However, our research distinctly emphasizes model training methodologies, as opposed to prompt engineering. 
% This focus is also instrumental in knowledge distillation, where insights from vast zero-shot LLMs are condensed into more efficient models, a primary subject of exploration in our work.

In summary, we offer the following principal contributions:
\vspace{-2mm}
\begin{itemize}
\item We introduce and formalize the task of structured entity extraction within the realm of closed information extraction.
% \item We curate and publicly release a dataset derived from Wikipedia, serving as a valuable resource for structured entity extraction research and applications.
\item We propose an evaluation metric with numerous variants tailored for assessing structured entity extraction.
\item We propose a new model leveraging the capabilities of large language models (LLMs), improving the effectiveness and efficiency for structured entity extraction.
\end{itemize}



% \begin{table}[t]
% \centering
% \caption{Differences between our Structured Entity Extraction (SEE) task and prior widely studied tasks.}
% \vspace{0.2cm}
% \label{tab:task-comparison}
% \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{c|cccc|c}
% \toprule
% Task & \makecell{Named Entity\\Recognition} & \makecell{Relation\\Recognition} & \makecell{Entity \\Linking} &
% \makecell{Local\\ Linking} & \makecell{External\\source}\\
% \midrule
% NER & \CheckmarkBold & - & - & - & - \\
% AmbER & - & - & \CheckmarkBold/- & -/\CheckmarkBold & KB/- \\
% oIE& \CheckmarkBold & \CheckmarkBold & - & - & - \\
% cIE & \CheckmarkBold & \CheckmarkBold & \CheckmarkBold & - & KB \\
% \midrule
% \textbf{SEE} & \CheckmarkBold & \CheckmarkBold & - & \CheckmarkBold& Ontology \\
% \bottomrule
% \end{tabular}}
% % \vspace{-0.5cm}
% \end{table}

==> section/02-related.tex <==
% \vspace{-4mm}
\section{Related work}
\label{sec:related}
\vspace{-2mm}
% \Ye{I need to revise the related work according to our new story line}
% First discuss IE has two categories
%
% Information extraction (IE) is the process of deriving structured semantic data from unstructured text~\cite{niklaus-etal-2018-survey}.
% %
% This process plays a crucial role in machine reading and comprehension.
% The output of IE significantly enhances various natural language processing (NLP) tasks, including question answering, search engine functionality, and the completion of knowledge graphs, ~\cite{liu2022open}.
%
In this section, we first review two different settings of information extraction tasks: open and closed.
%
We then explore how our task diverges from and intersects with existing information extraction endeavors.
% %
% The results of IE are instrumental in enhancing a variety of natural language processing (NLP) applications, including question answering systems, search engines, and the completion of knowledge graphs~\cite{han-etal-2020-data}.
%
% The process of transforming free text into structured knowledge is defined by knowledge base population~\cite{ji-grishman-2011-knowledge}, which aims to represent text information in the form of \textit{(entity1, relation, entity2)} fact triplets.
% %
% Several studies have centered on open information extraction (OIE)~\cite{oie2007banko}, in which the extracted triplets are in a free-text format.
% %
% The extracted relations are composed of selected words in input sentences,  producing one triple for every relation stated explicitly in the text, but is not required to infer implicit ones.
% %
% On the other hand, different research has been dedicated to closed information extraction (CIE)~\cite{josifoski2022genie}. 
% %
% This problem focuses on the extraction of comprehensive sets of fact triplets that conform to the constraints of relation or entity.
% %
% Several studies, such as \citet{dunn2022structured, walker2023extracting}, have explored the task of structured information extraction (sIE).
% %
% The key distinction in this formulation is that it yields structured records, like JSON documents, containing the necessary information, as opposed to producing a collection of triplets.

%
Open information extraction (OIE), initially introduced by \citet{oie2007banko}, aims to extract relational triplets from unstructured text, where entities and relations are directly sourced from input sentences.
%
The relations do not necessarily conform to a specific schema.
%
In contrast, closed information extraction (CIE) aims to extract facts from natural language that align with a pre-defined schema of relations or entities~\cite{josifoski2022genie}.

%
Our proposed structured entity extraction (SEE) operates within a closed setting, necessitating that all entity types and property keys adhere to a predefined schema. 
%
Unlike singular tasks such as named-entity recognition~\cite{li2020survey}, relation extraction~\cite{kumar2017survey}, and event extraction~\cite{li2022survey}, which focus on an individual aspect of information extraction, SEE undertakes to simultaneously address these three areas. 
%
It aims to comprehensively extract all entities, encompassing events and their associated properties.
%
Additionally, SEE encompasses coreference resolution~\cite{ stylianou2021neural, liu2023brief}, identifying when two mentions relate to the same entity.
%
This is crucial for aggregating all properties related to a single entity, as illustrated in the introduction section.
%
% While it shares similarities with entity linking~\cite{Angeli2015BootstrappedST}, it diverges in that only the relations should be mapped to a predefined schema, but the entities themselves may not strictly conform to the schema.
%
Given its multifaceted nature, SEE can be viewed as an integrated task that combines elements of named-entity recognition, entity-property extraction, relationship extraction, and coreference resolution. 
%
This integration allows for a more holistic approach to parsing and understanding structured information from unstructured texts.

%
Most existing works in information extraction focus on named-entity recognition and relation extraction.
%
TextRunner~\cite{yates-etal-2007-textrunner} has evolved unsupervised methods initially.
%
Recent advancements uses manual annotations, and Transformer-based models~\cite{roy-etal-2019-supervising, vasilkovsky2022detie, kolluru2020openie6}. 
%
Sequence generation techniques, such as IMoJIE~\cite{kolluru2020imojie} and GEN2OIE~\cite{kolluru-etal-2022-alignment}, have further refined OIE by transforming it into a sequence-to-sequence task~\cite{cui2018neural, lu2023pivoine}. 
%
Some other works, like GenIE~\cite{josifoski2022genie}, concentrate on a combination of named-entity recognition, relation extraction, and entity linking, where they assume a knowledge base is given. 
%
However, this assumption may not always hold, such as constructing a knowledge base from text.
%
Therefore, our proposed structured entity extraction has more practical assumptions and will be helpful for a lot of higher level tasks.

% %
% Structured entity extraction falls into the closed setting, where all property keys and entity types should follow a predefined schema.
% %
% Differing from named-entity recognition~\cite{li2020survey}, relation extraction~\cite{kumar2017survey}, and event extraction~\cite{li2022survey} along, structured entity extraction tries to finish these three tasks together.
% %
% It needs to extract all entities, including events, and all associated properties.
% %
% Differing from coreference resolution~\cite{ stylianou2021neural, liu2023brief} itself, structured entity extraction requires not only finding all expressions that refer to the same entity in a text but also extracting the relations inside these expressions.
% %
% Similar to entity linking~\cite{Angeli2015BootstrappedST}, structured entity extraction needs to align the extracted relations and entity types to a predefined schema, but the entity itself may not conform to any specific schema.
% %
% %
% With these differences and similarities, structured entity extraction is more like a combination of named-entity recognition, entity-property extraction, relationship extraction, and coreference resolution.

% OIE and CIE approaches have significantly advanced through direct and two-step extraction methods, and a step-by-step methodology, respectively. Direct extraction has evolved from TextRunner's unsupervised methods to sophisticated systems like SenseOIE, which uses manual annotations, and Transformer-based models like DetIE for triplet extraction. Sequence generation techniques and instruction tuning with LLMs, as seen in NeuralOIE and PIVOINE, have further refined OIE by transforming it into a sequence-to-sequence task. Two-step extraction methods employ advanced techniques, such as RnnOIE's BIO tagging with a Bi-LSTM transducer and Multi$^2$OIE's use of BERT embeddings. CIE's step-by-step methodology focuses on identifying entity mentions and their relations, often employing a pipeline of models including NER, EL, and RC. However, error propagation poses challenges, prompting the development of integrated end-to-end systems that improve performance by leveraging entity and relation data, utilizing methods ranging from multi-class classification to autoregressive models.


% %
% OIE has evolved through two primary approaches: direct extraction and a two-step extraction process.
% %
% Direct extraction methods originate from TextRunner~\cite{yates-etal-2007-textrunner}, which introduced an automated, unsupervised process. 
% %
% Recent advancements in this approach include SenseOIE~\cite{roy-etal-2019-supervising}, a system that enhances OpenIE extractions using various sources and manual annotations, DetIE~\cite{vasilkovsky2022detie}, a Transformer-based model labeling tokens for triplet extraction, and OpenIE6~\cite{kolluru2020openie6}, which employs an Iterative Grid Labeling (IGL) architecture.
% %
% In addition, sequence generation methods like NeuralOIE~\cite{cui2018neural} transform OIE into a sequence-to-sequence task, using coping strategies to minimize unknown tokens, while IMoJIE~\cite{kolluru2020imojie} iteratively adds extractions to the input sequence until an end token is reached.
% %
% PIVOINE~\cite{lu2023pivoine} achieves OIE by finetuning LLMs using instruction tuning.
% %
% For the two-step extraction process, methods like RnnOIE~\cite{stanovsky-etal-2018-supervised} and Multi$^2$OIE~\cite{Ro_2020} are notable. 
% %
% RnnOIE employs a BIO tagging scheme and a Bi-LSTM transducer, whereas Multi$^2$OIE utilizes BERT embeddings and multi-head attention for argument extraction. 
% %
% SpanOIE~\cite{zhan2019span} adopts a span-based technique, featuring separate modules for predicates and arguments, while the Logician model~\cite{sun2019logician} focuses on extracting triplets from Chinese text using language-specific heuristics and attention mechanisms.

% %
% CIE has predominantly pursued a step-by-step methodology, initially identifying entity mentions and their relations, followed by aligning these with elements in the pre-defined schema.
% %
% Another prevalent approach uses a pipeline of models, involving Named Entity Recognition (NER) for entity detection, Entity Linking (EL) for associating mentions with schema-specific entities, and Relation Classification (RC) to identify inter-entity relationships~\cite{canon2014Galarrage, Angeli2015BootstrappedST, chaganty-etal-2017-importance}. 
% %
% However, these methods often face challenges due to error propagation, impacting their effectiveness~\cite{mesquita-etal-2019-knowledgenet, trisedya-etal-2019-neural}.
% %
% To mitigate this, integrated end-to-end systems have been introduced, leveraging entity data to enhance relation extraction and vice versa, significantly boosting performance. 
% %
% Some utilize multi-class classification for ranking relations and entities~\cite{trisedya-etal-2019-neural, sui-etal-2021-set, liu2018seq2rdf}, while others like GenIE~\cite{josifoski2022genie} adopt an autoregressive method. 
%
% Unlike open information extraction (OIE), which generates triplets in free-text, CIE requires output triplets to match entities or relations in a pre-defined schema.

% \paragraph{Differences and Connections.}
% \Ye{Please help me confirm this part. @Haolun@Bhaskar}
% %
% Structured Entity Extraction expects JSON format outputs, while existing works predominately use triplets.
% %
% When using triplets, we know two relations corresponding to one same subject only if the extracted subjects' names are the same.
% Take the textual description we used in Figure.~\ref{fig:task} as an example.
% %
% If the extracted triplets are \textit{("Bill Gates", "is", "businessman")} and \textit{("Gates", "co-found", "Microsoft")}, we are unsure whether these two relations are referring to the same subject.
% %
% Therefore, it requires an additional disambiguation step, which is usually considered a separate task.
% %
% In contrast, JSON format omits this constraint, requiring model to implicitly learn whether two mentioned relations in the textual description are referring to the same subject.
%



% \subsection{Closed Information Extraction}
% %
% The objective of CIE is to comprehensively extract facts from natural language texts that adhere to a pre-defined relation or entity schema~\cite{josifoski2022genie}. 
% %
% Most current techniques tackle this challenge using a step-by-step approach.
% %
% One approach begins by identifying entity mentions and their interrelations within the raw text. 
% %
% This step is followed by a clarification process, where these entities and relations are aligned with their corresponding elements in the pre-defined schema.
% %
% Another strategy involves a sequential application of models for different tasks: (i) Named Entity Recognition (NER) to identify entity mentions, (ii) Entity Linking (EL) to associate these mentions with specific entities in the pre-defined schema, and (iii) Relation Classification (RC) to determine the relationships existing between these entities~\cite{canon2014Galarrage, Angeli2015BootstrappedST, chaganty-etal-2017-importance}.
% %
% However, due to their structured nature, these step-by-step methods suffer from the issue of error propagation, which significantly hampers their overall effectiveness~\cite{mesquita-etal-2019-knowledgenet, trisedya-etal-2019-neural}.
% %
% To overcome the issue of error propagation, integrated end-to-end systems have been developed for simultaneous extraction and clarification of entities and relations. 
% %
% These systems have the advantage of using entity data to enhance relation extraction and vice versa, leading to notable improvements in performance.
% %
% Some approaches use a method based on multi-class classification to rank relations and entities~\cite{trisedya-etal-2019-neural, sui-etal-2021-set, liu2018seq2rdf}. 
% %
% In contrast, others, like GenIE~\cite{josifoski2022genie}, employ autoregressive way for this purpose.
% %
% Closed information extraction (CIE) specifically demands that the elements of its output triplets, entities and relations, correspond with those in a pre-defined schema, whereas open information extraction (OIE) outputs triplets in free-text form. 

% \subsection{Structured Information Extraction}
% %
% Some types of information cannot be adequately captured through simple pairwise relationships between entities~\cite{dunn2022structured, walker2023extracting}. 
% %
% As an alternative, models are trained to produce structured records, such as JSON documents.
% %
% The benefit of this approach lies in its adaptability and accessibility~\cite{walker2023extracting}.
% %
% Virtually any information extraction task can be accommodated by creating a new output schema.
% %
% While in theory these JSON documents could be represented as triplets, fully cataloging all possible variations is not feasible in some cases~\cite{dunn2022structured}.
% %
% To address this challenge, \citet{dunn2022structured} and \citet{walker2023extracting} utilizes a pre-trained large language model (LLM), which is fine-tuned using a small set of prompt and completion pairs. 
% %
% This approach enables the extraction of information from individual sentences or across multiple sentences in abstracts or passages. 
% %
% The extracted information is then presented in a structured format, such as a list of JSON objects.

% \Ye{Discuss more about the connections and differences between our methods and existing works}

% \subsubsection{Tasks}
% \label{sec:related-task}

% \subsubsection{Approaches}
% \label{sec:related-approach}

% \bigskip\noindent
% Potential references: \citet{liu2020event, wadden2019entity, haghighi2010entity, shaowei2022survey, wang2021unire, zhang2017review, del2015methods, paass2023foundation, simoes2009information, grishman1997information}
